End-to-End Learned Early Classification of Time Series for In-Season Crop Type Mapping

Remote sensing satellites capture the cyclic dynamics of our Planet in regular time intervals recorded in satellite time series data. End-to-end trained deep learning models use this time series data to make predictions at a large scale, for instance, to produce up-to-date crop cover maps. Most time series classification approaches focus on the accuracy of predictions. However, the earliness of the prediction is also of great importance since coming to an early decision can make a crucial difference in time-sensitive applications. In this work, we present an End-to-End Learned Early Classification of Time Series (ELECTS) model that estimates a classification score and a probability of whether sufficient data has been observed to come to an early and still accurate decision. ELECTS is modular: any deep time series classification model can adopt the ELECTS conceptual idea by adding a second prediction head that outputs a probability of stopping the classification. The ELECTS loss function then optimizes the overall model on a balanced objective of earliness and accuracy. Our experiments on four crop classification datasets from Europe and Africa show that ELECTS allows reaching state-of-the-art accuracy while reducing the quantity of data massively to be downloaded, stored, and processed. The source code is available at https://github.com/marccoru/elects.

==> graphical_abstract.tex <==
	\textbf{Graphical Abstract}
	\vspace{4em}
	
	\includegraphics[width=\textwidth]{images/graphical_abstract2.pdf}


==> images/epsilon/archive/data/3 <==
ôc½:J=¾"Ï€¾j>w"¾2ύ¾*…–>'ݧ½wÍ6>0•=ߒM¾}½çº,ÿ<>»8>Ö¨4¾7×;TV"=·7>…(m½Rù>Öë>rE>"À½WV‹>̓M<ÃÓ='Ƚð"W¾‰!=Ãó<>O	¾£ 0½u…¾ñó'½Öoþ½ëQ>x€Ç½×Ó=ûÆQ>39;½@Z¾y¿¼¿Å=Ëòå=Ü^>ªeÂ=¸cä=±·½f¾\—V½
mº>ð®Ó=TÍr=Y¬a¾ñɾk뺻ï¥k>]o€>!C;=	'=½g$_¾)•?¾B¹&>A?x½

==> images/epsilon/archive/data/7 <==
¹@-Š™?4(¡?K›¿ïֈ?L¡>@¾áy¸>ZA_¿}vŠ?þ{®>tiž¿u¦ÿ?W¨®?-¿2¾ ö±½]5O¿Ô•"¿HpØ=yْ½å¾{>+‹?t°¾ç"}?
—¿ÏYj?MþT?â°½¿U½^¿î'Z?>VË¿ìx?¢´¿f[1?`?ݺÀÒ7#À©áp¿Ï󿿙~‰¿‡c¾ü_˜?TÁ?¥3ß?×Ì¿~…?sZ~?ãX?2Ÿ>Ž&»?Ò>=3·¿YG¢¿£?Ba@$‡¾¿5Ø>Ž^Q½|?ôg§?\3¾–p^¿V*?

==> related_work.tex <==

\section{Related Work}

\subsection{Early Time Series Classification}

The problem of early classification has been in focus in the time series classification community, as summarized in the review of Gupta \textit{et al.}~\cite{gupta2020approaches}.
In a seminal paper, Xing \textit{et al.} \cite{xing2012early} suggested in \emph{Early Classification on Time Series} (\textsc{ECTS}) to delay decision-making for a nearest-neighbor classifier until the neighborhood of the time series becomes stable over time. % to be classified
This idea of delaying the decision until the classifier is \emph{reliable} enough has been investigated in several other works.
Hatami \textit{et al.}~\cite{hatami2013classifiers} base their approach on an ensemble of classifiers for which a certain level of consensus has to be reached for the decision to be considered reliable.
\textsc{RelClass}~\cite{parrish2013classifying} waits until it is highly probable that the decision made using observation available up to time $t$ % $\xuptot$
is the same as the decision that would be made based on the entire time series.
Another example of this family of methods is \textsc{EDSC}~\cite{xing2011extracting} in which local features called \emph{shapelets}~\cite{ye2009time} are extracted based on their predictive power.
A later feature selection scheme is then used to select the shapelets that can predict both early and accurately.

One limitation of these methods is that they do not explicitly model the trade-off between earliness and accuracy.
To overcome this limitation, Martinez \textit{et al.}~\cite{martinez2018deep} cast the early classification problem into a reinforcement learning framework, while Dachraoui \textit{et al.} \cite{dachraoui2015early} proposed to include the cost of delaying the decision in the loss function.
In the latter work, clustering and cross-validation schemes are used to predict future classification costs.
From that information, a final decision is made only if it seems unlikely that the cost will decrease further in the future.
Tavenard \textit{et al.} \cite{tavenard2016cost} expanded this method by expressing the decision to delay a classification as a binary classification problem itself, therefore removing the need for data clustering in the process. Mori \textit{et al.}~\cite{mori2017early} also consider explicitly optimizing the trade-off between earliness and accuracy.
Their SR2-CF2 model variant first trains a Gaussian Process Classifier for each sub-sequence length independently. It then uses a genetic algorithm to find the parameter for a stopping rule that takes prediction confidence for each class into account.
While leading to promising results both in terms of accuracy and earliness, this results in a high computational complexity of $\mathcal{O}(N^2T^2)$ with $N$ time series examples of sequence length $T$.
Finally,  the TEASER algorithm~\cite{schafer2020teaser} casts early time series classification as a two-level classification problem. While a first classifier periodically predicts the incoming time series to compute class probabilities, a second classifier, a one-class SVM, processes these probabilities and predicts whether the predicted label is reliable enough. This second classifier is trained in a subsequent process where it is asked to predict whether to stop the classification on samples that were correctly classified by the first classifier. 
%In contrast to TEASER, our method performs both decision in a single stage with a shared feature extractor and two linear output heads. \devis{}{[I THINK THIS FINAL PARA OF CONTEXTUALISATION OF ELECTS IS NOT GOOD ENOUGH. YOU CANNOT JUST SAY IN CONTRAST WITH THE LAST ONE I REVIEWED, MINE IS DIFFERENT. TRY TO CONTEXTUALISE ELECTS WITH ALL THE METHODS IN ONE SENTENCE. WHAT DOES YOURS HAVE THAT IS UNIQUE? ]}

\subsection{In-season and Early Crop Type Mapping} % Early Crop Type Classification With Remote Sensing

The problem of early time series classification has been a steady topic of interest in remote sensing. In crop type mapping, it is often referred to as in-season or early crop type classification which can guide agro-economic decisions that could be made potentially months in advance.


\textbf{Incremental Classification}.
Most remote sensing approaches typically follow an incremental classification procedure, as termed by Inglada \textit{et al.}, \cite{inglada2016improved}. Here, a supervised classification is performed every time a new image becomes available. The prediction is based on the information provided by all previous images.
This poses the challenge of an increasing number of input features every time new data becomes available. Skakun \textit{et al.}~\cite{skakun2017early} avoided this issue by defining a sequence-length-invariant max-NDVI feature in combination with a Gaussian Mixture Model classifier.
A more popular strategy \cite{mcnairn2014early,vaudour2015early,inglada2016improved,cai2018high} involves re-fitting the classifier with the increased feature set.
Early work of McNairn \textit{et al.}~\cite{mcnairn2014early} classified an incrementally larger sequence of TerraSAR-X images in Canada with a decision tree for pasture, corn, soybean discrimination. While a single image achieved a solid classification base for corn of $70$\%, additional images in August and September improved the accuracy to above $90$\%. Vaudour \textit{et al.}~\cite{vaudour2015early} similarly studied the achievable classification accuracy with two Pleiades and one Spot image in early April in France with an SVM classifier. With more images, Inglada \textit{et al.}~\cite{inglada2016improved} studied the effect of increasing the sequence length on classification accuracy with $20$ Sentinel-1 and Landsat-$8$ images and a random forest classifier in southern France.
These approaches can be summarized as case studies for remote sensing experts to foresee the expected classification accuracy given a date of classification for specific regions and sets of target classes.
% \devis{}{[FIND A BETTER ARGUMENT THAN `MORE SYSTEMATICALLY (WHICH IS VERY PEJORATIVE). WHY IS THIS MORE SYSTEMATIC?]},
Cai \textit{et al.}~\cite{cai2018high} gathered $1`322$ Landsat scenes of one county in the US-Corn Belt between $2000$ and $2015$. For each time step, a $4$-layer Multi-Layer-Perceptron classifier was trained on specific sequence lengths of previous years and then tested on one target year.
Johnson \& Mueller~\cite{johnson2021pre} noted that in the early-season crop labels from the US Cropland Data Layer (CDL) \cite{boryan2011monitoring} from previous years were more predictive for the current year, due to systematic crop rotations, than early satellite observations alone.

\textbf{Cluster-then-Label}.
Konduri \textit{et al.}~\cite{konduri2020mapping} proposed an elegant but conceptually complex cluster-then-label strategy to avoid retraining models on new observations. They cluster MODIS NDVI time series of the entire United States into $5000$ phenoregions with a $k$-means based algorithm \cite{hargrove2004potential}. Some labeled pixels from CDL are used to assign crop labels to specific phenoregions. A partial time series of a test year can then be compared to the NDVI profile of each phenoregion, which does not require re-training a classification model.

\textbf{Low-dimensional Generative Distributions}.
Most recently, Lin \textit{et al.}~\cite{lin2021early} model the data distributions of corn and soybeans in a generative way in a specific two-dimensional spectral feature space of red-edge and short-wave infrared bands from archival data. They condition these distributions on time and sample training data of a given day of the year to train a date-specific classifier without labels from a target year.

\vspace{1em}

Our proposed ELECTS-trained Early Classification Model falls into the incremental classification category where a classification is made with new available data. In contrast, to existing early- and in-season classification methods~\cite{mcnairn2014early,vaudour2015early,inglada2016improved,cai2018high} it does not require re-training the classifier when new data is available. It is conceptually simpler to the cluster-than-label \cite{konduri2020mapping} and generative sampling and retraining \cite{lin2021early} strategies.


==> revieweranswers.tex <==
\noindent Subject: Revision of PHOTO-D-22-01154

\vspace{3em}

\noindent 
Dear Editor, Dear Reviewers

\vspace{3em}	

\noindent 
Thank you very much for your helpful and constructive feedback. We revised the manuscript according to your suggestions and provide point-by-point replies below.

\vspace{1em}
\noindent 
We hope that we could modify the manuscript to the reviewers' standards. 
In the attached manuscript, we indicate new text in blue.


\vspace{2em}

\noindent Sincerely,
\vspace{0.5em}

\noindent Marc Ru\ss{}wurm on behalf of the authors


\newpage

\noindent \textbf{Editor}

\begin{answer}{\noindent Both reviewers agree that this paper is technically sound and well-presented. However, Reviewer 1 has offered very useful feedback about streamlining the methodology section further. A major revision will be required to accomplish this.}{}
	Thank you for the summary of the paper and for giving us the chance to streamline the manuscript further. We have removed large sections from the introduction and Figure 1 to streamline the reading flow. We rearranged the results section, modified the title and subtitles, and provided a graphical abstract. 
	We answered the reviewers' remarks point-by-point below.
\end{answer}

\textbf{Reviewer 1}

\begin{answer}{In the previous review of the manuscript, both the relevance of the theme and the proposed model were highlighted, but several problems were pointed out. Compared to the previous submission, this manuscript version is more concise and understandable, even considering that the two datasets (located in Ghana and South Sudan) have been included to assess implementation flexibility.}{}
	We thank the reviewer for the accurate summary and for emphasizing the problem's relevance. We are glad that this manuscript version is considered "more concise and understandable" by R1 and "well-organized" by R2. Regarding the comments of this reviewer, we have extensively reworked the first submission and separated the experiments that justified model design decisions ($\alpha$ and $\varepsilon$ parameters) from results that are specific to the problem of crop type mapping. In this re-submission, we decided only to include the results and moved the parameterization and ablation studies to the appendix. 
	
	
	
\end{answer}

\begin{answer}{However, several adjustments are still necessary for the manuscript to clearly show the reach and scope of the tests performed and, thus, the potential of the ELECTS model. It is necessary to adjust, mainly the titles and subtitles of the methodology and results in subsections to the content covered.}{}
We thank the reviewer for the detailed suggestions, and we answer the modifications point-by-point below.
\end{answer}

\begin{answer}{Methodology: sections 3 (Data) and 4 (Implementation Details) should be included under Section 2 (Methodology). The methodology (or Material and Methods) section could contain:
		2. Materials and Methods
		2.1 Model (which would include the ELECTS loss function - contemplated in Figure 1)
		2.2 Datasets
		2.3 Implementation Details
		2.4 Model Evaluation}{}
	
	We thank the reviewer for suggesting re-organizing the Methods and Data sections.
	
	We understand that merging data and method in a combined Material and Methods section is useful in many applied problems where the presented method is intimately connected to the respective dataset, e.g., through problem-specific feature design or preprocessing. 
	We largely followed the reviewer's suggestions and streamlined and reorganized the Methods section: we integrated the Implementation Details section in the Methodology as the third subsection. As it references the datasets, we moved the "Datasets" section (formerly "Data") before the Methodology. This enabled us to remove the last sentence in the introduction that anticipated some takeaways from the following sections.
	However, we decided not to merge the methodology and data sections. We would like to emphasize that our ELECTS model and loss function is general enough to be applied to other time series problems. As the methodology can be understood independently from the dataset, we decided not to merge (and thus connect) the dataset and methodology sections in a combined Materials and Methods section.
 	
	The new order in this revision is now 2. Datasets, 3. Methodology, 3.1 Model, 3.2 ELECTS loss function, 3.3 Implementation Details, 3.4 Model evaluation, and 4. Results.
	
\end{answer}

\begin{answer}{In addition, it would be desirable to add the last subsection dealing with the evaluation of the model. The datasets have already been presented, but an overview of the tests performed (and with which subsets) has not been contemplated. This appears in results but in a pulverized form.}{}
We added a Model Evaluation subsection to the Methodology where we outline the training and testing split procedure for each dataset. We also mention once that the model configuration (hyper-parameters) is kept identical throughout all experiments, which avoids the need to re-state this fact in the results section.

We have explicitly added the Dataset names to the introductory paragraph of the Results that provides an overview of the tests performed. We hope that this clarifies what datasets have been used for the respective results.
\end{answer}

\begin{answer}{Results: presentation of results is very confusing, mixed with methodology and analysis. It is necessary that the headings of sections and subsections highlight the model's ability to result in earliness and accuracy, as well as its ability to handle datasets of different locations and characteristics.}{}
	We have improved and streamlined the headings of the subsections, as detailed in the following answers. We also refined the text throughout the entire results section and hope that the presentation of the results is now less confusing.
\end{answer}

\begin{answer}{The title of subsection 5.1, "Classification Process and Accuracy of the Fields Parcels stopped by ELECTS" is generic and vague. }{}
	We thank the reviewer for pointing this out and renamed this section from "Classification Process and Accuracy of the Field Parcels stopped by ELECTS" to "Accuracy Evaluation".
\end{answer}

\begin{answer}{The results could be divided into two more general sections, and then the relevant content could be inserted. For example:
	3. Experimental Results
}{}
	We have rearranged the results section. However, we would prefer to maintain the section title "Results" and not rename it to "Experimental Results", as suggested. We adopted a semantic difference between "Experiments" and "Results" in this work: we see ``Experiments'' as the experimental evaluations of the Method, i.e., the model design and the loss function, comparison to one other early classification model, and accuracy-only methods. The ``Results'' section in this work is more application-focused and evaluates the model performance (measured in accuracy and earliness) concerning the crop type mapping problem. We believe that mixing the methods-focused "experiments" (now in the appendix) and the application-focused "results" caused major confusion in the previous submission. This is why we focus only on ``Results'' on crop type mapping problems in this work and moved the method-focused experimental evaluations into the appendix. We hope the choice is reasonable from the reviewer`s perspective.
\end{answer}

\begin{answer}{3.1 ELECTS Performance - which would include assessments carried out in the Brittany study area (3.1.1. Single Field Prediction; 3.1.2. Classification of Fields at Different Times; 3.1.3. Quantitative Prediction Accuracy; 3.1.4. Influence of the Stopping Times, instead of Analysis)}{}
	We acknowledge that the subsection titles are too generic and do not reflect this detail, as outlined by the reviewer.
	This is why we renamed "Classification Process and Accuracy of the Field Parcels stopped by ELECTS" to "Accuracy Evaluation" and "Analyses of the stopping times" to "Earliness Evaluation" to emphasize this distinction.
	
	We thank the reviewer for suggesting merging accuracy and earliness results into a single performance section.
	We would like to emphasize that the performance of early classification models has the two distinct components of "accuracy" and "earliness" that we aimed to evaluate in different subsections (formerly "Classification Process and Accuracy of the Field Parcels stopped by ELECTS" and "Analyses of the stopping times"). This is why we would like to avoid merging these two aspects of performance into a single subsection, "3.1 ELECTS Performance", as proposed by the reviewer.
\end{answer}

\begin{answer}{3.2 Generalization Capability of the Model (or Flexibility of the ELECTS Model, or.., etc.) - which would include the current sub-items 5.3.1 and 5.3.2.
		Of course, the previous considerations are only suggestions for reorganizing the topic content and adapting the titles to the content. Any changes that meet these criteria are acceptable.}{}
	
	Thanks to the reviewer's comment, we added "of ELECTS" to "Applicability across datasets" for clarity.
		
	We have discussed the word "generalization" in the title of Section 4.3 (formerly "Applicability across datasets" 5.3) internally before this re-submission.
	We would like to avoid the word generalization, as, in the context of different geographic areas, it implies training and testing on different regions, which we do not do in this work. We \emph{apply} the model to different areas but still train on available datasets there. This is why we believe that Applicability is more suitable than "Generalization" or "Flexibility".
\end{answer}

\begin{answer}{Furthermore, some specific points identified in the manuscript should be revised by the authors:}{}
	We thank the reviewer for the detailed feedback and address the points below.
\end{answer}

\begin{answer}{Page 2 - lines 1-25: Figure 1 is unnecessary. The preliminary description of ELECTS in the Introduction is enough.}{}
	We removed the figure and introduced a similar one as a graphical abstract, as also suggested by R2. We also removed all references to this figure in the introduction and results in sections.
\end{answer}

\begin{answer}{Page 3 - excess of information about apparently disconnected aspects. It is necessary to adjust the text, connecting these aspects with the scientific gap.
	}{}
	We thank the reviewer for pointing this out. We revised the introduction and removed the second large paragraph that appeared misplaced after describing related work.
\end{answer}

\begin{answer}{Page 5 - Figure 2: the functions associated with Eq. (2) and Eq. (3) are inverted in the figure.
	}{}
	We thank the reviewer for pointing out this mistake! We fixed the annotations to equations in this figure.
\end{answer}

\begin{answer}{Page 11 - Figure 5 caption: the caption of a figure must be direct. Needless to say, "This Figure illustrates...". If it's a figure, it illustrates something.}{}
	We thank the reviewer for this comment. We removed the introductory sentence "this figure illustrates" as it is unnecessary. 
\end{answer}

\begin{answer}{Page 12 - lines 291-292: The statement "The model predictions did not vary noticeably in June 21st (third row in Figure 5)" is unclear. This image indicates that the prediction did not vary significantly from what? Or does this refer to accuracy?}{}
	The accuracy in this sentence refers to the ratio of blue/correct and red/incorrect fields in the third row and second column of Figure 4 in comparison to the first column (April 12th) that was discussed in the previous sentence. At the same time, the model stops the classification for an increasing number of fields (indicated in black in the fourth row).
	
	We thank the reviewer for pointing out that this association to the previous time step (April 12th) is not very clear. We now added "concerning April $12$th" to this sentence to make this relationship clearer. 
\end{answer}

\begin{answer}{Page 14 - Figure 7: each part ("a" and "b") of this figure has its own caption in addition to the general caption. This needs to be revised.}{}
	We thank the reviewer for pointing out the content overlap between the subcaptions and the main caption. We revised the main caption to be more general and left a detailed description of the figure in the subcaptions.
\end{answer}

\begin{answer}{- Some figures incorporate explanations and analyses into the legend which go further than what is indicated in the figure itself. You can do that in the text.}{}
	We refined and reworked all captions in this revision and gladly shorten and refined the captions further if it is a requirement.
\end{answer}

\begin{answer}{- Standardize throughout the text how to refer to classes (uppercase, lowercase, italics, etc.). As long as a single style is adopted.}{}
	We fixed the missed style modifications in the class names. We made a further pass in the paper and homogenized the style of classnames.
\end{answer}

\begin{answer}{Please note that some of the above considerations were pointed out in the previous review. That is, several problems persist in this new version, which must be carefully considered by the authors.}{}
	We thank the reviewer again for the  detailed review and comments on our work. We hope to have clarified and addressed all reviewer comments in this revision.
	We hope to have clarified and addressed the points raised in this revision.
	We are happy to address any further points that the reviewer thinks may not have been addressed previously.
\end{answer}

\newpage
\textbf{Reviewer 2}


\begin{answer}{Reviewer 2: This paper presents an End-to-End Learned Early Classification (ELECTS) method for early and accurate classification of various crop-type datasets. This work is of great importance to risk management. The paper is well-organized, and the methods and results are sound. But there are several small issues to be addressed.
	}{}
	We thank the reviewer for acknowledging the importance of early classification for several problems, e.g. risk management. 
	We integrated and answer the three suggestions below.
\end{answer}


\begin{answer}{1. The title should be more specific since this paper focuses on crop classification.}{}
	We acknowledge that the title should be more specific, we modified the title now to "End-to-End Learned Early Classification of Time Series \textbf{for In-Season Crop Type Mapping}" to address this issue.
\end{answer}

\begin{answer}{2. It is suggested to provide a graphic abstract or workflow by including the data, methods, and results to demonstrate the overall framework of this paper.}{}
	We thank the reviewer for pointing out the benefit of a graphical abstract. We removed figure 1 (remark by R1) and added a graphical abstract to the paper that includes both a schematic (former Figure 1) and the plots from the data example shown in Fig 3.
\end{answer}

\begin{answer}{3. It is suggested to cut down some text in section 2.1. For example, the description and equations for RNN and LSTM, which are widely known and not the key improvement of the paper, could be concise.}{}
	We agree that known relationships should not be restated. However, we emphasize that we already present a shortened high-level description of the LSTM equation that does not include the internal gates.
	Furthermore, we had the impression that some general properties of LSTMs (e.g., that they can classify a variable length time series) was not clear to reviewers in the previous submission of this paper. This is why we decided to keep the general equations of RNN and LSTM in the paper. 
	
	We thank the reviewer for his precise and constructive comments.
\end{answer}



